On Classification Thresholds for Graph Attention with Edge Features

The recent years we have seen the rise of graph neural networks for prediction tasks on graphs. One of the dominant architectures is graph attention due to its ability to make predictions using weighted edge features and not only node features. In this paper we analyze, theoretically and empirically, graph attention networks and their ability of correctly labelling nodes in a classic classification task. More specifically, we study the performance of graph attention on the classic contextual stochastic block model (CSBM). In CSBM the nodes and edge features are obtained from a mixture of Gaussians and the edges from a stochastic block model. We consider a general graph attention mechanism that takes random edge features as input to determine the attention coefficients. We study two cases, in the first one, when the edge features are noisy, we prove that the majority of the attention coefficients are up to a constant uniform. This allows us to prove that graph attention with edge features is not better than simple graph convolution for achieving perfect node classification. Second, we prove that when the edge features are clean graph attention can distinguish intra- from inter-edges and this makes graph attention better than classic graph convolution.

==> On Classification Thresholds for Graph Attention with Edge Features (arXiv)/00_abstract.tex <==
\begin{abstract}
% \fontsize{10pt}{12pt}\selectfont

The recent years we have seen the rise of graph neural networks for prediction tasks on graphs. One of the dominant architectures is graph attention due to its ability to make predictions using weighted edge features and not only node features. In this paper we analyze, theoretically and empirically, graph attention networks and their ability of correctly labelling nodes in a classic classification task. More specifically, we study the performance of graph attention on the classic contextual stochastic block model (CSBM). In CSBM the nodes and edge
features are obtained from a mixture of Gaussians and the edges from a stochastic block model. We consider a general graph attention mechanism that takes random edge features as input to determine the attention coefficients. We study two cases, in the first one, when the edge features are noisy, we prove that the majority of the attention coefficients are up to a constant uniform. This allows us to prove that graph attention with edge features is not better than simple graph convolution for achieving perfect node classification. Second, we prove that when the edge features are clean graph attention can distinguish intra- from inter-edges and this makes graph attention better than classic graph convolution. %We further support our theoretical findings with experiments.

%The recent years we have seen the rise of graph neural networks for prediction tasks on graphs. One of the dominant architectures is graph attention due to its ability to make predictions using the weighted edge features and not just the features of the node itself. In this paper we examine the performance of graph attention on a simple synthetic data model called the contextual stochastic block model (CSBM). In CSBM the nodes and edge\footnote{Note that the original definition of the CSBM or other papers that utilize the CSBM do not include edge features. We keep the same name of the model since the name is sufficiently general.} features are obtained from a mixture of Gaussians and the edges from a stochastic block model. We consider a simple but general graph attention mechanism that takes random edge features as input to determine the attention coefficients. We study two cases, in the first one, when the edge features are noisy, we prove that the majority of the attention coefficients are up to a constant uniform. This allows us to prove that graph attention with edge features is not better than simple graph convolution for achieving perfect node classification. Second, we prove that when the edge features are clean graph attention can discriminate intra- from inter-edges and this makes graph attention better than graph convolution, however, it does not outperform a simple unsupervised method that only uses the graph and ignores the node features. We further support our theoretical findings with synthetic experiments on the CSBM.

\end{abstract}

==> On Classification Thresholds for Graph Attention with Edge Features (arXiv)/01_introduction.tex <==
\section{Introduction}\label{sec:intro}

Learning from multi-modal datasets is currently one of the most prominent topics in artificial intelligence. The reason behind this trend is that many applications, such as recommendation systems, fraud detection and vision, require some combination of different types of data. 
% In addition, it is often the case that data exhibit correlations which need to be captured for downstream applications. 
In this paper we are interested in multi-modal data which combine a graph, i.e., a set of nodes and edges, with attributes for each node and edge. The attributes of the nodes/edges capture information about the nodes/edges themselves, while the edges among the nodes capture relations among the nodes. Capturing relations is particularly helpful for applications where we are trying to make predictions for nodes given neighborhood data. 

One of the most prominent ways of handling multi-modal data for downstream tasks such as node classification are graph neural networks~\cite{GMS05,scarselli:gnn,BZSL14,DMAGHAA15,HBL15,AT16,DBV16,HYL17,kipf:gcn}. Graph neural network models can mix hand-crafted or automatically learned attributes about the nodes while taking into account relational information among the nodes. Their output vector representation contains both global and local information for the nodes. This contrasts with neural networks that only learn from the attributes of entities. 

\subsection{Motivation and goals}
Graph neural networks have found a plethora of uses in chemistry~\cite{gilmer:quantum, scarselli:gnn}, biology, and in various industrial applications. Some representative examples include fighting spam and abusive behaviors, providing personalization for the users~\cite{YHCEHL18}, and predicting states of physical objects~\cite{battaglia:graphnets}. Given wide applicability and exploding popularity of GNNs, theoretically understanding in which regimes they work best is of paramount importance.

One of the most popular graph neural network architectures is the Graph Attention Network (GAT). Graph attention~\cite{Velickovic2018GraphAN} is usually defined as
averaging the features of a node with the features of its neighbors by appropriately weighting the edges of a graph before spatially convolving the node features. It is generally expected by practitioners that GAT is able to downweight unimportant edges and set a large weight for important edges, depending on the downstream task. In this paper we analyze the graph attention mechanism. %We focus on understanding if practitioners' intuition about graph attention is true on a simple synthetic setting. 
% We show rigorously when Graph Attention Network outperform classic Graph Convolution Network on node classification. 
%We complement our positive results with an in depth-analysis of foundational limits of graph attention for achieving perfect classification.
%We study settings where this intuition is correct, and we focus on understanding foundational limits of graph attention for achieving perfect classification. 

We focus on node classification, which is one of the most popular tasks for graph learning. We perform our analysis using the contextual stochastic block model (CSBM)~\cite{BVR17,DSM18}. The CSBM is a coupling of the stochastic block model (SBM) with a Gaussian mixture model. We focus on two classes where the answer to the above question is sufficiently precise to understand the performance of graph attention and build useful intuition about it.

We study perfect classification as it is one of the three questions that has been asked for the community detection for SBM without node features~\cite{Abbe2018}. We leave results on other types of classification guarantees for future work. Our goal is study the performance of graph attention on a well-studied synthetic data model. We see our paper as a small step in the direction of building theoretically justified intuition about graph attention and better attention mechanisms.

\subsection{Contributions} 
We study the performance of graph attention with edge and node features for the CSBM. The edge features follow a Gaussian mixture model with two means, one for intra-edges and one for inter-edges. We call the edge features clean when the distance between the means is larger than the standard deviation. We call the edge features noisy when the distance between the means is smaller than the standard deviation. We split our results into two parts. In the first part we consider the case where the edge features that are passed to the attention mechanism are clean. In the second part we consider the case where the edge features are noisy. We describe our contributions below.

\begin{enumerate}
    \item \textit{Separation of intra and inter attention coefficients for clean edge features}. There exists an attention architecture which can distinguish intra- from inter-edges. This attention architecture allows us to prove that the means of the convolved data do not move closer, while achieving large variance reduction. It also allows us to prove that the threshold of perfect node classification for graph attention is better than that of graph convolution.
    \item \textit{Perfect node classification for clean edge features}. Let $\sigma$ be the standard deviation of the node features, $n$ the number of nodes and $p,q$ the intra- and inter-edge probabilities. If the distance between the means of the node features is $\omega\left(\sigma \sqrt{\frac{\log{n}}{n \max(p,q)}}\right)$. Then with high probability graph attention classifies the data perfectly.
    \item \textit{Failure of perfect node classification for clean edge features}. If the distance between the means of the node features is small, that is smaller than $K \sigma  \sqrt{\frac{\log{n}}{n\max(p,q)}\left(1-\max(p,q)\right)}$ for some constant $K$, then graph attention can't classify the nodes perfectly with probability at least $1-1/n^{1-\max(p,q)}$.
    \item \textit{Uniform intra and inter attention coefficients for noisy edge features.} We prove that for $n-o(n)$ nodes at least $90\%$ of their attention coefficients are up to a constant uniform. This means that a lot of attention coefficients are up to a constant the same as those of graph convolution. This property allows us to show that in this regime graph attention is not better than graph convolution.
    \item \textit{Perfect node classification for noisy edge features.} If the distance is $ \omega\left(\sigma\frac{p+q}{|p-q|}\sqrt{\frac{\log n}{n\max(p,q)}}\right)$, then with high probability graph attention classifies all nodes correctly. 
    \item \textit{Failure of perfect node classification for noisy edge features.} If the distance is less than $K\sigma\frac{p+q}{|p-q|}\sqrt{\frac{\log n}{n\max(p,q)}(1-\max(p,q))}$ for some constant $K$, then graph attention can't classify the nodes perfectly with probability at least $1-1/n^{1-\max(p,q)}$.
\end{enumerate}

Finally we complement our theoretical results with an empirical analysis confirming our main findings.


==> On Classification Thresholds for Graph Attention with Edge Features (arXiv)/02_previous_work.tex <==
\section{Relevant Work}\label{sec:prev_work}

There have been numerous papers proposing new graph neural network architectures that is impossible to acknowledge all works in one paper. We leave this work for relevant books and survey papers on graph neural networks, examples include~\cite{HamilBook,WPCLZY21}. From a theoretical perspective, a few authors have analyzed graph neural networks using traditional machine learning frameworks or from a signal processing perspective~\cite{CLB19,Chien:2020:joint,Zhu:2020:generalizing,XHLJ19,GJJ20,A2020,ALoukas2020}. For a recent survey in this direction see the recent survey paper~\cite{J22} that focuses on three main categories, representation, generalization and extrapolation. In our paper we analyze graph attention from a statistical perspective that allows us to formally understand claims about graph attention. 

In the past, researchers have put significant effort in understanding community detection for the SBM~\cite{Abbe2018}. Usually the results for community detection are divided in three parameters regimes for the SBM. The first type of guarantee that was investigated was that of exact recovery or perfect classification. 
We are also interested in perfect node classification, but our work is on graph attention for the CSBM.
The analysis of exact recovery in SBM and perfect classification in CSBM for graph attention are significantly different. In fact, our focus is not on designing the best algorithm for the exact classification task but it is on understanding the advantages and limitation of Graph Attention over other standard architectures. As a consequence, the model we analyze is a non-linear function of the input data since we have to deal with the coupling of highly nonlinear attention coefficients, the node features and the graph structure. 

A closely related work is~\cite{BFJ2021}, which studies the performance of graph convolution~\cite{kipf:gcn} on CSBM as a semi-supervised learning problem. In our paper we work with graph attention and we compare it to graph convolution. Another relevant work is~\cite{fountoulakis2022graph}. In this paper the authors also study the performance of graph attention for CSBM. However, in~\cite{fountoulakis2022graph} edge features are not used and there is no result provided about when graph attention fails to achieve perfect node classification, only a conjecture is provided. In this paper we provide a complete treatment regarding the question of perfect classification when edge features are given. Another paper that studies performance of graph attention on CSBM is~\cite{anonymous2023results}. In this paper the attention architecture is constructed using ground-truth labels and it is fixed. The authors also consider an attention architecture which is constructed using an eigenvector of the adjacency matrix when the community structure in the graph can be exactly recovered. Thus in~\cite{anonymous2023results} only a rather optimistic scenario is studied, that is, when we are given a good attention architecture. In our paper, we consider the case where additional edge features are given that follow a Gaussian mixture model and we analyze the performance of graph attention when these features are clean or noisy. We provide complete analysis about the attention coefficients, instead of assuming them, and we show how they affect perfect node classification when the edge features are clean or noisy.

Within the context of random graphs another relevant work is~\cite{KBV21,MLLK22}. In the former paper, the authors study universality of graph neural networks on random graphs. In the latter paper the authors go a step further and prove that the generalization error of graph neural networks between the training set and the true distribution is small, and the error decreases with respect to the number of training samples and the average number of nodes in the graphs. In our paper we are interested in understanding the parameters regimes of CSBM such that graph attention classifies or fails to classify the data perfectly. This allows us to compare the performance of graph attention to other basic approaches such as a graph convolution. 

Other papers that have studied the performance of graph attention are~\cite{BAY21,KTA19,hou2019measuring}. In~\cite{BAY21} the authors show that graph attention fails due to a global ranking of nodes that is generated by the attention mechanism in~\cite{Velickovic2018GraphAN}. They propose a deeper attention mechanism as a solution. Our analysis a deeper attention mechanism is not required since we consider independently distributed edge features and the issue mentioned in~\cite{BAY21} is avoided.

The work in~\cite{KTA19} is an empirical study of the ability of graph attention to generalize on larger, complex, and noisy graphs. Finally, in~\cite{hou2019measuring} the authors propose a different metric to generate the attention coefficients and show empirically that it has an advantage over the original GAT architecture. In our paper we consider the original and most popular attention mechanism~\cite{Velickovic2018GraphAN} and its deeper variation as well.

==> On Classification Thresholds for Graph Attention with Edge Features (arXiv)/03_notation.tex <==
\section{Preliminaries}\label{sec:notation}

In this section we describe the data model that we use and the graph attention architecture.

\subsection{The contextual stochastic block model with random edge features}

In this section we describe the CSBM~\cite{DSM18}, which is a simple coupling of a stochastic block model with a Gaussian mixture model. Let $(\epsilon_{k})_{k\in[n]}$ be i.i.d \ Bernoulli random variables. These variables define the class membership of the nodes. In particular, consider a stochastic block model consisting of two classes
$C_{0}=\{i\in[n]:\epsilon_{i}=0\}$ and $C_{1}=C_{0}^c$ with inter-class edge probability $q$ and intra-class edge probability $p$ with no self-loops\footnote{In practice, self-loops are often added to the graph and the following adjacency matrix $\tilde{A}$ is used instead: $\tilde{A}=(\tilde{a}_{ij})$ is the matrix $A + I$ and $D$ to be the diagonal degree matrix for $\tilde{A}$, so that $D_{ii} = \sum_{j\in[n]}\tilde{a}_{ij}$ for all $i\in[n]$. Our results can be extended to this case with minor changes.}.
In particular, given $(\epsilon_{k})$ the adjacency matrix $A=(a_{ij})$ follows a Bernoulli distribution where $a_{ij}\sim \Ber(p)$ if $i,j$ are in the same class  and $a_{ij}\sim \Ber(q)$ if they are in distinct classes. This completes the distributions for the class membership and the graph. Let us now describe the distributions for the node and edges features.

Consider the node features $x_{i}$ to be independent $d$-dimensional Gaussian random vectors with
$x_{i}\sim N(\mu,\sigma I)$ if $i\in C_{0}$ and
$x_{i}\sim N(-\mu,\sigma I)$ if $i\in C_{1}$.
Here $\mu\in\R^{d}$ is the mean, $\sigma\ge 0$ is the standard deviation and $I$ is the identity matrix. 
Let $\mathcal{E}$ be the set of edges which consists of pairs $(i,j)$ such that $a_{ij}=1$. Consider $E\in\R^{|\mathcal{E}|\times h}$ to be the edge feature matrix such that such that each row $E_{(i,j)}$ is an independent $h$-dimensional Gaussian random vector with
$E_{(i,j)}\sim N(\nu,\zeta I)$ if $(i,j)$ is an intra-edge, i.e., $i,j\in C_{0}$ or $i,j\in C_{1}$, and
$E_{(i,j)}\sim N(-\nu,\zeta I)$ if $(i,j)$ is an inter-edge, i.e., $i\in C_{0}, j\in C_1$ or $i\in C_{1}, j\in C_0$.
Here $\nu\in\R^{d}$ is the mean, $\zeta\ge 0$ is the standard deviation.

Denote by $CSBM(n,p,q,\mu,\nu,\sigma, \zeta)$ the coupling of a stochastic block model with the Gaussian mixture models for the nodes and the edges with means $\mu,\nu$ and standard deviation $\sigma,\zeta$, respectively, as described above. We denote a sample by $(A,X, E)\sim CSBM(n,p,q,\mu,\nu,\sigma, \zeta)$.

\subsection{Assumptions}
We now we state two standard assumptions on the CSBM that we will use in our analysis. The first assumption is $p,q\ge \Omega (\log^2 n / n )$, and it guarantees that the expected degrees of the graph are $\Omega(\log^2 n)$, they also guarantee degree concentration. The second assumption is that the standard deviation $\zeta$ of the edge features is constant. This assumption is without loss of generality since all that really matters is the ratio of the distance between the means of the edges features over the standard deviation. As long as we allow the distance between the means to grow while $\zeta$ is fixed then the results are not restricted, while the analysis is simplified.

\subsection{Graph attention}

The graph attention convolution is defined as $\hat x_i=\sum_{j\in [n]} \tilde{A}_{ij}\gamma_{ij} x_j$ $\forall i\in[n]$, 
where $\gamma_{ij}$ is the attention coefficient of the edge $(i,j)$. We focus on a single layer graph attention since this architecture is enough for the simple CSBM that we consider. 
%This means that we consider classifying the convolved data $\tilde{x}_i$ with a learnable linear classifier $w\in\R^{d}$.

There are many ways to set the attention coefficients $\gamma$. We discuss the setting in our paper and how it is related to the original definition in~\cite{Velickovic2018GraphAN} and newer ones~\cite{BAY21}. We define the attention function $\Psi(E_{(i,j)})$ which takes as input the features of the edge $(i,j)$ $E_{(i,j)}$ and outputs a scalar value. The function $\Psi$ is often parameterized by learnable variables, and it is used to define the attention coefficients
\begin{align*}
    \gamma_{ij}:= \frac{\exp(\Psi(E_{(i,j)}))}{\sum_{\ell\in N_i}\exp(\Psi(E_{(i,\ell)}))}\label{def:attention_coeff},
\end{align*}
where $N_i$ is the set of neighbors of node $i$. 

In the original paper~\cite{Velickovic2018GraphAN} the function $\Psi$ is a linear function of the two dimensional vector $[w^T x_i,w^T x_j]$ passed through LeakyRelu, where the coefficients of the linear function are learnable parameters, $w$ are learnable parameters as well and are shared with the parameters outside attention. In this paper we consider independent edge features as input to the attention mechanism. Although in the original paper~\cite{Velickovic2018GraphAN} edge features are mentioned as an input to the model this seems an important departure from what was extensively studied in~\cite{Velickovic2018GraphAN}. However, using edge features captures the effect of dominating noise in graph attention, which is what we are interested in this paper for understanding performance of graph attention. 
%We also perform extensively experiments to demonstrate that this gap in analysis is not important. 
Finally, we consider $\Psi$ functions that are a composition of a Lipschitz and a linear function. This is enough to prove that graph attention is able to distinguish intra- from inter-edges and consequently leads to better performance than graph convolution when the edge features are clean. Given that the edge features in our data model are independent from node features, this setting avoids the issues discussed in~\cite{BAY21}.


% $\Psi$ function is constructed as a linear function of the input, since this is enough to prove that graph attention is able to distinguish intra- from inter-edges that also results to better performance than graph convolution. While in \textcolor{red}{blah} we consider any function $\Psi$ that is realized by an MLP.

% In this paper we do not limit ourselves to the original setting only. For the positive perfect classification results we construct an attention function that is a generalized version of the original where $\Psi$ is realized by an MLP. This is enough for the positive results since all its needed is to show that there exist a graph attention architecture that achieves perfect classification. For the negative results we utilize the edge features only and we ignore the node features. This seems a rather strong limitation. However, ignoring the model still captures the effect of dominating noise in graph attention. Also, this attention architecture allows us to treat the attention independently of the node features. We also perform extensively experiments to demonstrate that this gap in analysis is not important.


% A one layer multi-head graph attention convolution~\cite{Velickovic2018GraphAN} uses $K\in \N$ weight matrices $\bW^1,\ldots, \bW^K\in \R^{F\times F'}$ and averages their individual (single-head) outputs. We consider the most simplified case of a single graph attention layer (i.e., $F'=d$ and $F=1$), since this is enough to demonstrate the concepts that we want for the CSBM described above.

==> On Classification Thresholds for Graph Attention with Edge Features (arXiv)/04_results.tex <==
\section{Results}\label{sec:results}

In this section we describe our results. We split the section into two parts. In the first part we describe performance of graph attention in case the edge features are clean. In the second part we describe performance of graph attention in case the edge features are noisy.

\subsection{Clean edge features}

Consider the case of clean edge features, this means that $\|\nu\|\ge \omega(\zeta \sqrt{\log (|\mathcal{E}|)})$. We call this regime clean because in this case there is not much overlap between the two Gaussians in the Gaussian mixture model of the CSBM. In the following theorem we prove that there exists an attention architecture such that it is able to distinguish intra- from inter-edges. The reason that such an attention architecture is useful is because it allows us to prove in~\cref{thm:clean} that the means of the convolved node features do not move closer, while achieving large variance reduction. The importance of such an attention mechanism is also verified by the fact that using it the threshold of perfect node classification in~\cref{thm:clean} is better than that of graph convolution. We comment on this later on in this section.

\begin{proposition}\label{prop:gammas}
Let $(A,X, E)\sim CSBM$, and assume that $\|\nu\|\ge \omega(\zeta \sqrt{\log (|\mathcal{E}|)})$. If $p>q$, we have that there exists a function $\Psi$ that provides the following attention coefficients
    \begin{equation*}
    \gamma_{ij}=
        \begin{cases}
            \frac{2}{n p}(1\pm o_n(1)) & i,j\in C_0 \mbox{ or } i,j\in C_1\\
            o\left(\frac{1}{n(p+q)}\right) & \mbox{otherwise.}\\
        \end{cases}
    \end{equation*}
    with probability $1-o_{n}(1)$. If $q>p$, we have that
    \begin{equation*}
    \gamma_{ij}=
        \begin{cases}
            o\left(\frac{1}{n(p+q)}\right) & i,j\in C_0 \mbox{ or } i,j\in C_1\\
            \frac{2}{n q}(1\pm o_n(1)) & \mbox{otherwise.}\\
        \end{cases}
    \end{equation*}
    with probability $1-o_{n}(1)$.
\end{proposition}

\textit{Proof sketch}. We construct $\Psi$ such that it separates intra- from inter-edges and it concentrates around its mean. We define $s:=\sign(p-q)\nu/\|\nu\|$ and  $\Psi(E_{(i,j)}):= s^T E_{(i,j)}$, which measures correlations with one of the means of the Gaussian mixture for the edge features. If $p>q$ the $\Psi$ function concentrates around a large positive value for intra-edges and a large negative value for inter-edges. The opposite holds for $q>p$. Then we plug in $\Psi$ in the definition of the attention coefficients $\gamma_{ij}$. Using concentration of $\Psi$ we prove the result.

In the following theorem we utilize~\cref{prop:gammas} to prove a positive result and a negative result for perfect classification using graph attention. 

\begin{theorem}\label{thm:clean}
Let $(A,X, E)\sim CSBM$, and assume that $\|\nu\|\ge \omega(\zeta \sqrt{\log (|\mathcal{E}|)})$.
\begin{enumerate}
    \item If $\|\mu\|\ge \omega\left(\sigma \sqrt{\frac{\log{n}}{n \max(p,q)}}\right)$, then we can construct a graph attention architecture that classifies the nodes perfectly with probability $1-o_n(1)$.
    \item If $\|\mu\|\le  K \sigma  \sqrt{\frac{\log{n}}{n\max(p,q)}\left(1-\max(p,q)\right)}$ for some constant $K$ and if $\max(p,q) \le 1-36 \log n / n$, then for any fixed $\|w\|=1$ graph attention fails to perfectly classify the nodes with probability at least $1-2\exp(-c'(1-\max(p,q))\log n)$ for some constant $c'$.
\end{enumerate}
\end{theorem}

\textit{Proof sketch}. For part 1 we use the attention coefficients from~\cref{prop:gammas} and we plug them in the definition of graph attention. Then because the distance between the means is large we can use simple concentration arguments to show that the convolved data concentrate around their means, which are classifiable with high probability using the classifier $w:=\sign(p-q)\mu/\|\mu\|$. This classifier measures correlation with one of the means. For part 2, the Gaussian noise dominates the means of the convolved node features. Thus there exists at least one node for which is not possible to detect its correct class with the given probability. 

\textit{Discussion of~\cref{thm:clean}}. There is a difference between the threshold in the positive result (part 1 of~\cref{thm:clean}) and the negative result (part 2 of~\cref{thm:clean}). The difference is prominent when $\max(p,q)=1-o_n(1)$. In that case, the threshold for the negative regime is very small and the probability can be so low that the result is not meaningful. This is an expected outcome. Consider the case $p=1$ and $q$ very small, then after convolution the data collapse approximately to two points that can be easily separated with a linear classifier. The difference between the two thresholds is small when $\max(p,q) \le 1 - \epsilon$ for any constant $\epsilon\in(0,1)$. That is, when $\max(p,q)$ is away from $1$. Finally, there is a difference due to $\omega$ in the positive result. This difference is not important since we can make the order in $\omega$ small with the cost of affecting the probability of perfect classification, although the probability will still be $1-o_n(1)$.

A limitation of our analysis is the assumption of a fixed $w$. Although in the proof of part 1 we utilize a specific fixed $w$ and we show that for this fixed $w$ graph attention is able to perfectly classify the nodes, it would be an interesting future work to set $w$ to be the optimal solution of some expected loss function.

It is important to note that if the edge features are clean then graph attention is better than graph convolution. In~\cref{thm:noisy} we will see that the threshold for graph convolution for the perfect classification is $\|\mu\| = \omega\left(\frac{p+q}{|p-q|}\sqrt{\frac{\log n}{n\max(p,q)}}\right)$, while for failing perfect classification the threshold is $\|\mu\| \le K\sigma \frac{p+q}{|p-q|}\sqrt{\frac{\log n}{n\max(p,q)}(1-\max(p,q))}$ for some constant $K$. By simply comparing these thresholds to those of graph attention in~\cref{thm:clean} it is easy to see that the parameter regime of CSBM where graph attention can perfectly classify the data is larger than that of graph convolution. First the difference $|p-q|$ is not affecting graph attention and also the threshold on the distance between the means is smaller for graph attention.%\footnote{Lastly, we note that even in the regime where the edge features are clean graph attention does not outperform a simple spectral method that only uses the adjacency matrix $A$. We are referring to the method of thresholding the second principal eigenvector of the adjacency matrix $A$~\cite{Abbe2018}. In particular, in Theorem 13 in~\cite{Abbe2018} it is claimed that thresholding the second principal eigenvector of $A$ detects the class of all nodes correctly with high probability if $|\sqrt{p}-\sqrt{q}|> \sqrt{2 \log n}/n$. On the other hand, if this condition holds for the SBM then graph attention will fail to classify the nodes perfectly if the distance between the means is small, i.e., the condition in part 2 of~\cref{thm:clean} holds. However, it is also important to note that if $|\sqrt{p}-\sqrt{q}|\le \sqrt{2 \log n}/n$, then graph attention will classify the nodes perfectly if the distance between the means is large, i.e., the condition in part 1 of~\cref{thm:clean} holds, while the simple spectral method that we mentioned above will fail to classify the node perfectly. Therefore, depending on the parameter regime of CSBM, graph attention is worse or better than a simple spectral method.}

\subsection{Noisy edge features}\label{ssec:noisy-edge-features}

Consider the case of noisy edge features, this means that $\|\nu\|\le K \zeta$ for some constant $K$. We call this regime noisy because in this case there is a lot of overlap between the two Gaussians in the Gaussian mixture model of the CSBM. Note that there is a gap between this regime and the clean features regime, the two regimes differ by a factor of $\omega(\sqrt{\log (|\mathcal{E}|)})$. Although this factor grows with $|\mathcal{E}|$ we note that the factor changes very slowly with $|\mathcal{E}|$. For example, for $|\mathcal{E}|=10^{20}$, $\sqrt{\log (|\mathcal{E}|)}\approx 6.78$. Below we present the result about $\gamma$, which is crucial for obtaining node classification results and whose proof is deferred to the Appendix.

\begin{proposition}\label{prop:gammas_noisy}
Assume that $\|\nu\| \le K \zeta$ for some constant $K$. Then, with probability at least $1-o_n(1)$, there exists a subset of nodes $\mathcal{A} \subseteq [n]$ with cardinality at least $n - o(n)$ such that for all $i \in \mathcal{A}$ the following hold:
\begin{enumerate}
	\item There is a subset $J_{i,0} \subseteq N_i \cap C_0$ with cardinality at least $\frac{9}{10}|N_i \cap C_0|$, such that $\gamma_{ij} = \Theta(1/|N_i|)$ for all $j \in J_{i,0}$;
	\item There is a subset $J_{i,1} \subseteq N_i \cap C_1$ with cardinality at least $\frac{9}{10}|N_i \cap C_1|$, such that $\gamma_{ij} = \Theta(1/|N_i|)$ for all $j \in J_{i,1}$.
\end{enumerate}
\end{proposition}

%\textit{Proof sketch}. \textcolor{red}{blah}

The above proposition states that for the majority of the nodes at least $90\%$ of their intra- and inter-edge attention coefficients are up to a constant uniform. This behaviour is similar to that of GCN. We utilize~\cref{prop:gammas_noisy} in the next theorem to prove that graph attention performs similarly to graph convolution.

\begin{theorem}\label{thm:noisy}
Let $(A,X, E)\sim CSBM$, and assume that $\|\nu\| \le K \zeta$ for some constant $K$.
\begin{enumerate}
    \item If $\|\mu\| = \omega\left(\sigma\frac{p+q}{|p-q|}\sqrt{\frac{\log n}{n\max(p,q)}}\right)$, with probability $1-o_n(1)$ graph attention classifies all nodes correctly.
    \item If $\|\mu\| \le K' \sigma \frac{p+q}{|p-q|}\sqrt{\frac{\log n}{n\max(p,q)}(1-\max(p,q))}$ for some constant $K'$  and if $\max(p,q) \le 1-36 \log n / n$, then for any fixed $\|w\| = 1$ graph attention fails to perfectly classify the nodes with probability at least $1-2\exp(-c'(1-\max(p,q))\log n)$ for some constant $c'$.
\end{enumerate}
\end{theorem}

\textit{Proof sketch}. 
The sketch of the proof of this theorem is similar to~\cref{thm:clean}. The major difference is that when the edge features are noisy the majority of the attention coefficients are up to a constant uniform, see~\cref{prop:gammas_noisy}, and the attention mechanism is not able to distinguish intra- from inter-edges. Let's start the sketch for part 2. Using~\cref{prop:gammas_noisy} we prove that the convolved means of the node features get closer by $(p+q)/(p-q)$. That's how this quantity appears in the thresholds. Again, using concentration arguments for the noise in the data and the assumed bound on the distance between the means we can show that the noise is larger than the convolved means with high probability. Therefore, graph attention misclassifies at least one node with high probability. The proof for part 1 is easy, we simply pick a function $\Psi$ that allows us  to match the threshold in part 2. This is achieved by simply setting $\Psi=0$, which also happens to reduce graph attention to graph convolution since all attention coefficients are exactly uniform. Because the attention coefficients are uniform the term $n(p+q)$ appears in the threshold. The remaining of the proof follows the same approach as part 1 of~\cref{thm:clean}.

% For part 1 we use the attention coefficients from~\cref{prop:gammas_noisy} and we plug them in the definition of graph attention. Then because of the distance between the means is large we can use simple concentration arguments to show that the convolved data concentrate around it their mean, which are classifiable with high probability using the classifier $w:=\sign(p-q)\mu/\|\mu\|$. This classifier measures correlation with one of the means. For part 2 we show that the Gaussian noise dominates the means of the convolved node features with the given probability. Thus there exists at least one node for which is not possible to detect its correct class with the given probability. 

\textit{Discussion on~\cref{thm:noisy}}. Note that the same thresholds hold for graph convolution\footnote{The analysis for graph convolution is nearly identical to~\cref{thm:noisy}. Graph convolution has also been analyzed in~\cite{BFJ2021}, but our analysis includes the dependence on $p,q$, while in~\cite{BFJ2021} the authors consider $(p-q)/(p+q)$ to be a constant. Moreover, the analysis in our paper holds regardless of $p>q$ or $q>p$.}. 
Therefore, we conclude that graph attention is not better than graph convolution for perfect node classification when the edge features are noisy. %Additionally, when the edge features are noisy graph attention is not better than the simple spectral method of thresholding the principal eigenvector of $A$. In particular, our comments about comparison graph attention to the simple spectral method are the same as in the case where the edge features are clean.

%  In particular, if $\min\{p,q\} \le 1 - \epsilon$ for some small constant $\epsilon > 0$ then $\Lambda(n,p,q) = \Omega(1)$ and $\Delta(n,p,q) = \Omega(1)$.

%Let us first discuss the gap between the thresholds in part 1 and part 2 in~\cref{thm:noisy}. If $\min\{p,q\} \le 1 - \epsilon$ for some small constant $\epsilon > 0$ then $\Lambda(n,p,q) = \Omega(1)$ and $\Delta(n,p,q) = \Omega(1)$. Plugging in $\Lambda(n,p,q)$ and $\Delta(n,p,q)$ in the threshold of part 2 and the corresponding probability we get that the threshold is up to a constant factor similar to the threshold of part 1, while the probability becomes $1-o_n(1)$. However, if $\epsilon=o_n(1)$, for an appropriate rate in $o_n(1)$, the gap could be potentially high, and the probability could also be meaningless. However, in practice, it is enough to assume that $\epsilon$ is a small positive constant.

==> On Classification Thresholds for Graph Attention with Edge Features (arXiv)/05_conclusion.tex <==
\section{Conclusion}
We study conditions on the parameter of the CSBM with edge features such that graph attention can achieve or fail perfect node classification. We split our results into two parts. The first part is when the edge features are clean and the second part is when the edge features are noisy. If the edge features are clean we show that graph attention is able to distinguish intra from inter attention coefficients which allows us to prove that the condition for perfect classification is better than that of graph convolution. If the edge features are noisy we show that the majority of attention coefficients are up to a constant uniform which then implies that graph attention performs similarly to graph convolution.

Working with synthetic data models has a lot of limitations due to their gap with real data, but they also have very important advantages such as providing a solid insight about the performance of methods. It is more productive to discuss limitations in our analysis for potential future researchers who might wish to extend the present work. A limitation of our analysis is the assumption of a fixed $w$ for our negative results. It would be interesting future work to set $w$ to be the optimal solution of some expected loss function. Finally, it would be interesting to study the performance of methods beyond perfect classification.

==> On Classification Thresholds for Graph Attention with Edge Features (arXiv)/A2_experiments.tex <==
\section{More experiments on real data}

In~\cref{a-table:1} and~\cref{a-table:2} we present the results for all classes for the data in the main paper. 

\begin{table}[ht!]
\caption{Percentages of intra- and inter-mass (intra-m and inter-m respectively) allocation for graph attention (GA) and graph convolution (GC), and test accuracy. We illustrate results for class $0$ and $1$ of each dataset, the rest are shown in the appendix. The first two rows of each dataset correspond to class $0$ and the latter to correspond to class $1$.} \vspace{0.1cm}
\centering
 \begin{tabular}{||c | c c c c c ||} 
 \hline
 data & class & method & intra-m & inter-m  & acc.\\ [0.5ex] 
 \hline\hline
\multirow{20}{*}{\rotatebox[origin=c]{90}{Amzn Co.}} & \multirow{2}{*}{$0$} & GC & $98.7$ & $1.3$ & $96.8$ \\
& & GA & $98.1$ & $1.9$ & $96.7$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $93.6$ & $6.4$ & $91.4$ \\
& & GA & $93.3$ & $6.7$ & $88.7$ \\ \cline{2-6}
& \multirow{2}{*}{$2$} & GC & $98.1$ & $1.9$ & $95.8$ \\
& & GA & $97.8$ & $2.2$ & $92.1$ \\ \cline{2-6}
& \multirow{2}{*}{$3$} & GC & $97.5$ & $2.5$ & $96.0$ \\
& & GA & $96.0$ & $4.0$ & $96.0$ \\ \cline{2-6}
& \multirow{2}{*}{$4$} & GC & $89.4$ & $10.6$ & $89.7$ \\
& & GA & $89.4$ & $10.6$ & $83.3$ \\ \cline{2-6}
& \multirow{2}{*}{$5$} & GC & $99.6$ & $0.4$ & $97.8$ \\
& & GA & $99.5$ & $0.5$ & $98.0$ \\ \cline{2-6}
& \multirow{2}{*}{$6$} & GC & $97.0$ & $3.0$ & $96.4$ \\
& & GA & $96.5$ & $3.5$ & $96.5$ \\ \cline{2-6}
& \multirow{2}{*}{$7$} & GC & $99.1$ & $0.9$ & $96.8$ \\
& & GA & $98.5$ & $1.5$ & $94.9$ \\ \cline{2-6}
& \multirow{2}{*}{$8$} & GC & $91.8$ & $8.2$ & $88.9$ \\
& & GA & $91.7$ & $8.3$ & $86.5$ \\ \cline{2-6}
& \multirow{2}{*}{$9$} & GC & $99.3$ & $0.7$ & $97.9$ \\
& & GA & $99.0$ & $1.0$ & $98.2$ \\
\hline \hline
\multirow{16}{*}{\rotatebox[origin=c]{90}{Amzn Ph.}} & \multirow{2}{*}{$0$} & GC & $99.0$ & $1.0$ & $95.1$ \\
& & GA & $98.8$ & $1.2$ & $96.0$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $94.9$ & $5.1$ & $94.2$ \\
& & GA & $95.5$ & $4.5$ & $89.0$ \\ \cline{2-6}
& \multirow{2}{*}{$2$} & GC & $99.4$ & $0.6$ & $96.5$ \\
& & GA & $99.1$ & $0.9$ & $92.8$ \\ \cline{2-6}
& \multirow{2}{*}{$3$} & GC & $93.6$ & $6.4$ & $91.5$ \\
& & GA & $91.5$ & $8.5$ & $88.6$ \\ \cline{2-6}
& \multirow{2}{*}{$4$} & GC & $96.2$ & $3.8$ & $88.4$ \\
& & GA & $94.5$ & $5.5$ & $88.6$ \\ \cline{2-6}
& \multirow{2}{*}{$5$} & GC & $99.7$ & $0.3$ & $98.6$ \\
& & GA & $99.6$ & $0.4$ & $95.1$ \\ \cline{2-6}
& \multirow{2}{*}{$6$} & GC & $94.3$ & $5.7$ & $86.8$ \\
& & GA & $92.7$ & $7.3$ & $82.4$ \\ \cline{2-6}
& \multirow{2}{*}{$7$} & GC & $95.7$ & $4.3$ & $95.5$ \\
& & GA & $94.0$ & $6.0$ & $95.5$ \\
\hline
\end{tabular}
\label{a-table:1}
\end{table}

\begin{table}[ht!]
\caption{Percentages of intra- and inter-mass (intra-m and inter-m respectively) allocation for graph attention (GA) and graph convolution (GC), and test accuracy. We illustrate results for class $0$ and $1$ of each dataset, the rest are shown in the appendix. The first two rows of each dataset correspond to class $0$ and the latter to correspond to class $1$.} \vspace{0.1cm}
\centering
 \begin{tabular}{||c | c c c c c ||} 
 \hline
 data & class & method & intra-m & inter-m  & acc.\\ [0.5ex] 
 \hline\hline
\multirow{14}{*}{\rotatebox[origin=c]{90}{Cora}} & \multirow{2}{*}{$0$} & GC & $94.2$ & $5.8$ & $89.5$ \\
& & GA & $94.7$ & $5.3$ & $88.6$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $97.3$ & $2.7$ & $92.3$ \\
& & GA & $97.4$ & $2.6$ & $93.7$ \\ \cline{2-6}
& \multirow{2}{*}{$2$} & GC & $97.9$ & $2.1$ & $86.9$ \\
& & GA & $98.1$ & $1.9$ & $90.8$ \\ \cline{2-6}
& \multirow{2}{*}{$3$} & GC & $93.6$ & $6.4$ & $70.7$ \\
& & GA & $94.1$ & $5.9$ & $73.3$ \\ \cline{2-6}
& \multirow{2}{*}{$4$} & GC & $96.3$ & $3.7$ & $88.8$ \\
& & GA & $96.6$ & $3.4$ & $88.8$ \\ \cline{2-6}
& \multirow{2}{*}{$5$} & GC & $96.8$ & $3.2$ & $91.7$ \\
& & GA & $96.7$ & $3.3$ & $91.3$ \\ \cline{2-6}
& \multirow{2}{*}{$6$} & GC & $98.1$ & $1.9$ & $94.9$ \\
& & GA & $98.2$ & $1.8$ & $95.1$ \\
\hline \hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{PubMed}} & \multirow{2}{*}{$0$} & GC & $92.2$ & $7.8$ & $82.1$ \\
& & GA & $92.1$ & $7.9$ & $82.8$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $91.4$ & $8.6$ & $58.8$ \\
& & GA & $90.6$ & $9.4$ & $59.5$ \\ \cline{2-6}
& \multirow{2}{*}{$2$} & GC & $89.4$ & $10.6$ & $60.8$ \\
& & GA & $89.1$ & $10.9$ & $61.8$ \\
\hline \hline
\multirow{12}{*}{\rotatebox[origin=c]{90}{CiteSeer}} & \multirow{2}{*}{$0$} & GC & $94.3$ & $5.7$ & $92.0$ \\
& & GA & $94.4$ & $5.6$ & $91.6$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $92.6$ & $7.4$ & $82.6$ \\
& & GA & $92.8$ & $7.2$ & $82.8$ \\ \cline{2-6}
& \multirow{2}{*}{$2$} & GC & $92.3$ & $7.7$ & $86.2$ \\
& & GA & $92.7$ & $7.3$ & $85.2$ \\ \cline{2-6}
& \multirow{2}{*}{$3$} & GC & $93.9$ & $6.1$ & $80.0$ \\
& & GA & $93.8$ & $6.2$ & $78.4$ \\ \cline{2-6}
& \multirow{2}{*}{$4$} & GC & $94.7$ & $5.3$ & $85.9$ \\
& & GA & $94.9$ & $5.1$ & $84.9$ \\ \cline{2-6}
& \multirow{2}{*}{$5$} & GC & $96.2$ & $3.8$ & $86.5$ \\
& & GA & $96.1$ & $3.9$ & $85.7$ \\
\hline
\end{tabular}
\label{a-table:2}
\end{table}

\section{Experiments on real data without edge features}

In the real experiments in the main paper we split the features of the dataset into half. The first half is used for node features and the second half is used for edge features. This leaves a small gap compared to the main setting in the original paper~\cite{Velickovic2018GraphAN} and also in our Preliminaries section in the main paper. Here we re-do the same experiments but without splitting the features and using the original setting in~\cite{Velickovic2018GraphAN}. The results are given in~\cref{a-table:3} and~\cref{a-table:4}. The results and the conclusion are similar in this setting as well.

\begin{table}[ht!]
\caption{Percentages of intra- and inter-mass (intra-m and inter-m respectively) allocation for graph attention (GA) and graph convolution (GC), and test accuracy. We illustrate results for class $0$ and $1$ of each dataset, the rest are shown in the appendix. The first two rows of each dataset correspond to class $0$ and the latter to correspond to class $1$.} \vspace{0.1cm}
\centering
 \begin{tabular}{||c | c c c c c ||} 
 \hline
 data & class & method & intra-m & inter-m  & acc.\\ [0.5ex] 
 \hline\hline
\multirow{20}{*}{\rotatebox[origin=c]{90}{computers}} & \multirow{2}{*}{$0$} & GC & $98.7$ & $1.3$ & $96.8$ \\
& & GA & $98.5$ & $1.5$ & $96.9$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $93.6$ & $6.4$ & $91.7$ \\
& & GA & $94.5$ & $5.5$ & $91.7$ \\ \cline{2-6}
& \multirow{2}{*}{$2$} & GC & $98.1$ & $1.9$ & $97.5$ \\
& & GA & $98.1$ & $1.9$ & $97.1$ \\ \cline{2-6}
& \multirow{2}{*}{$3$} & GC & $97.5$ & $2.5$ & $96.0$ \\
& & GA & $97.1$ & $2.9$ & $96.0$ \\ \cline{2-6}
& \multirow{2}{*}{$4$} & GC & $89.4$ & $10.6$ & $90.3$ \\
& & GA & $90.7$ & $9.3$ & $86.5$ \\ \cline{2-6}
& \multirow{2}{*}{$5$} & GC & $99.6$ & $0.4$ & $98.7$ \\
& & GA & $99.6$ & $0.4$ & $98.6$ \\ \cline{2-6}
& \multirow{2}{*}{$6$} & GC & $97.0$ & $3.0$ & $96.4$ \\
& & GA & $97.2$ & $2.8$ & $96.4$ \\ \cline{2-6}
& \multirow{2}{*}{$7$} & GC & $99.1$ & $0.9$ & $97.7$ \\
& & GA & $98.8$ & $1.2$ & $97.1$ \\ \cline{2-6}
& \multirow{2}{*}{$8$} & GC & $91.8$ & $8.2$ & $91.5$ \\
& & GA & $93.2$ & $6.8$ & $90.7$ \\ \cline{2-6}
& \multirow{2}{*}{$9$} & GC & $99.3$ & $0.7$ & $98.2$ \\
& & GA & $99.2$ & $0.8$ & $98.3$ \\
\hline \hline
\multirow{16}{*}{\rotatebox[origin=c]{90}{photo}} & \multirow{2}{*}{$0$} & GC & $99.0$ & $1.0$ & $95.3$ \\
& & GA & $98.9$ & $1.1$ & $95.6$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $94.9$ & $5.1$ & $95.6$ \\
& & GA & $95.2$ & $4.8$ & $91.2$ \\ \cline{2-6}
& \multirow{2}{*}{$2$} & GC & $99.4$ & $0.6$ & $96.9$ \\
& & GA & $99.3$ & $0.7$ & $96.9$ \\ \cline{2-6}
& \multirow{2}{*}{$3$} & GC & $93.6$ & $6.4$ & $92.3$ \\
& & GA & $94.1$ & $5.9$ & $91.4$ \\ \cline{2-6}
& \multirow{2}{*}{$4$} & GC & $96.2$ & $3.8$ & $96.1$ \\
& & GA & $96.5$ & $3.5$ & $94.2$ \\ \cline{2-6}
& \multirow{2}{*}{$5$} & GC & $99.7$ & $0.3$ & $97.5$ \\
& & GA & $99.7$ & $0.3$ & $98.3$ \\ \cline{2-6}
& \multirow{2}{*}{$6$} & GC & $94.3$ & $5.7$ & $95.5$ \\
& & GA & $95.2$ & $4.8$ & $91.1$ \\ \cline{2-6}
& \multirow{2}{*}{$7$} & GC & $95.7$ & $4.3$ & $95.7$ \\
& & GA & $96.1$ & $3.9$ & $95.6$ \\
\hline
\end{tabular}
\label{a-table:3}
\end{table}

\begin{table}[ht!]
\caption{Percentages of intra- and inter-mass (intra-m and inter-m respectively) allocation for graph attention (GA) and graph convolution (GC), and test accuracy. We illustrate results for class $0$ and $1$ of each dataset, the rest are shown in the appendix. The first two rows of each dataset correspond to class $0$ and the latter to correspond to class $1$.} \vspace{0.1cm}
\centering
 \begin{tabular}{||c | c c c c c ||} 
 \hline
 data & class & method & intra-m & inter-m  & acc.\\ [0.5ex] 
 \hline\hline
\multirow{14}{*}{\rotatebox[origin=c]{90}{Cora}} & \multirow{2}{*}{$0$} & GC & $94.2$ & $5.8$ & $90.3$ \\
& & GA & $94.7$ & $5.3$ & $89.8$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $97.3$ & $2.7$ & $94.2$ \\
& & GA & $97.7$ & $2.3$ & $94.2$ \\ \cline{2-6}
& \multirow{2}{*}{$2$} & GC & $97.9$ & $2.1$ & $90.3$ \\
& & GA & $98.1$ & $1.9$ & $91.1$ \\ \cline{2-6}
& \multirow{2}{*}{$3$} & GC & $93.6$ & $6.4$ & $74.9$ \\
& & GA & $94.1$ & $5.9$ & $79.7$ \\ \cline{2-6}
& \multirow{2}{*}{$4$} & GC & $96.3$ & $3.7$ & $89.4$ \\
& & GA & $96.6$ & $3.4$ & $90.5$ \\ \cline{2-6}
& \multirow{2}{*}{$5$} & GC & $96.8$ & $3.2$ & $93.0$ \\
& & GA & $96.7$ & $3.3$ & $92.7$ \\ \cline{2-6}
& \multirow{2}{*}{$6$} & GC & $98.1$ & $1.9$ & $95.2$ \\
& & GA & $98.4$ & $1.6$ & $95.4$ \\
\hline \hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{PubMed}} & \multirow{2}{*}{$0$} & GC & $92.2$ & $7.8$ & $84.3$ \\
& & GA & $92.0$ & $8.0$ & $85.7$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $91.4$ & $8.6$ & $59.1$ \\
& & GA & $90.8$ & $9.2$ & $64.1$ \\ \cline{2-6}
& \multirow{2}{*}{$2$} & GC & $89.4$ & $10.6$ & $61.5$ \\
& & GA & $89.0$ & $11.0$ & $61.6$ \\
\hline \hline
\multirow{12}{*}{\rotatebox[origin=c]{90}{CiteSeer}} & \multirow{2}{*}{$0$} & GC & $94.3$ & $5.7$ & $92.7$ \\
& & GA & $94.3$ & $5.7$ & $92.3$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $92.6$ & $7.4$ & $83.2$ \\
& & GA & $93.1$ & $6.9$ & $83.8$ \\ \cline{2-6}
& \multirow{2}{*}{$2$} & GC & $92.3$ & $7.7$ & $85.7$ \\
& & GA & $92.7$ & $7.3$ & $85.7$ \\ \cline{2-6}
& \multirow{2}{*}{$3$} & GC & $93.9$ & $6.1$ & $79.6$ \\
& & GA & $93.9$ & $6.1$ & $79.8$ \\ \cline{2-6}
& \multirow{2}{*}{$4$} & GC & $94.7$ & $5.3$ & $87.5$ \\
& & GA & $94.6$ & $5.4$ & $87.3$ \\ \cline{2-6}
& \multirow{2}{*}{$5$} & GC & $96.2$ & $3.8$ & $87.6$ \\
& & GA & $96.3$ & $3.7$ & $88.2$ \\
\hline
\end{tabular}
\label{a-table:4}
\end{table}

==> On Classification Thresholds for Graph Attention with Edge Features (arXiv)/commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\newcommand{\std}{\operatorname{{\bf std}}}
%\newcommand{\Var}{\operatorname{{\bf Var}}}
%\newcommand{\Cov}{\operatorname{{\bf Cov}}}
\newcommand{\Varx}{\mathop{{\bf Var}\/}}
%\newcommand{\E}{\operatorname{{\bf E}}}
\newcommand{\Ex}{\mathop{{\bf E}\/}}
\renewcommand{\Pr}{\operatorname{{\bf Pr}}}
\newcommand{\Prx}{\mathop{{\bf Pr}\/}}
\newcommand{\Bin}{\operatorname{Bin}}
\newcommand{\Ber}{\operatorname{Ber}}
\newcommand{\poly}{\mathrm{poly}}
%\newcommand{\R}{\mathbbm R}

\newcommand{\N}{\mathbbm N}

%\newcommand{\eps}{\epsilon}

\newcommand{\ind}{{\bf 1}}

\newcommand{\bzero}{{\bf 0}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}


\newcommand{\boldf}{\boldsymbol{f}} % \bf taken
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
%\newcommand{\bm}{\boldsymbol{m}}
\newcommand{\boldn}{\boldsymbol{n}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\boldr}{\boldsymbol{r}} % \br taken
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}

\newcommand{\boldR}{\boldsymbol{R}}

\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bell}{\boldsymbol{\ell}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\btau}{\boldsymbol{\tau}} 
\newcommand{\brho}{{\boldsymbol{\rho}} }
\newcommand{\bgamma}{{\boldsymbol{\gamma}} }
\newcommand{\bphi}{{\boldsymbol{\varphi}} }
\newcommand{\bchi}{\boldsymbol{\chi}}
\newcommand{\beps}{\boldsymbol{\eps}}
\newcommand{\boldeta}{\boldsymbol{\eta}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\bvsigma}{{\boldsymbol{\varsigma}} }
\newcommand{\bvrho}{{\boldsymbol{\varrho}}}

\newcommand{\bGamma}{{\mathbf{\Gamma}} }
\newcommand{\bDelta}{\mathbf{\Delta}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\calbE}{\boldsymbol{\calE}}
\newcommand{\CSBM}{\textsf{CSBM}}
\newcommand{\LeakyRelu}{\mathrm{LeakyRelu}}
\newcommand{\indi}{\boldsymbol{1}}
\newcommand{\eqdef}{\stackrel{\rm def}{=}}
%\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newtheorem{theorem}{Theorem}
 \newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}[lemma]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{fact}[lemma]{Fact}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{question}{Question}
\newtheorem{problem}{Problem}
\newtheorem{openproblem}{Open Problem}
\newtheorem{goal}{Goal}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{assumption}{Assumption}

\newtheorem{definition}[lemma]{Definition}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{proposition*}{Proposition}
% non-italicized environments
%\theoremstyle{definition}%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}[theorem]{Remark}
\newtheorem{observation}[lemma]{Observation}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}
%\theoremstyle{plain}
\newcommand{\anote}[1]{{{\bf \color{blue} \; Amit: {#1}}}}
\newcommand{\subf}[2]{%
  {\small\begin{tabular}[t]{@{}c@{}}
  #1\\#2
  \end{tabular}}%
}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

==> On Classification Thresholds for Graph Attention with Edge Features (arXiv)/experiments.tex <==
\section{Synthetic Experiments}

We investigate empirically our theoretical results on the CSBM. We do $50$ trials and we present averaged results and standard deviation. In each trial we generate data $(A,X,E)$ that follow the CSBM. We use the constructed solutions that are described in our theorems, which come with the corresponding guarantees, to define the learnable parameters in the models. In particular, for the graph attention we set $w=\sign(p-q)\mu/\|\mu\|$. The attention function $\Psi$ is set to $\Psi(E_{(i,j)}):= s^T E_{(i,j)}$, where $s:=\sign(p-q)\nu/\|\nu\|$. For GCN we also set $w=\sign(p-q)\mu/\|\mu\|$. Furthermore, we set $n=400$, $d=n/\log^2 n$, $\sigma=0.1$ and each class has $n/2$ nodes.

\subsection{Clean edge features}

We set $\zeta=0.1$ and we pick the mean of the edge features $\nu$ such that $\|\nu\|\ge 100 \zeta \sqrt{\log (0.5n^2(p+q))}$.

\textbf{Varying $q$.} We perform two experiments to demonstrate parts 1 and 2 of~\cref{thm:clean}, For part 1, which is the positive result, we pick $\mu$ such that $\|\mu\| = 5\sigma \sqrt{\log n / (n\max(p,q))}$. For part 2, which is the negative result, we set $\|\mu\| = \sigma \sqrt{\log n / (n\max(p,q))}$. We fix $p=0.4$ and we vary $q$ from $\log^2/n$ to $2p$. In~\cref{fig:clean_edges_varying_q_positive} we present the positive result for graph attention and we also compare graph attention to graph convolution. For any value of $q$ graph attention achieves perfect classification while graph convolution depends on $|p-q|$. In~\cref{fig:clean_edges_varying_q_negative} we present the negative result for graph attention. In this experiment the distance between the means is small and graph attention fails to achieve perfect classification, but it is better than graph convolution.
 \begin{figure}[ht!]
      \centering
      \begin{subfigure}[b]{0.49\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{figures/clean_edges_varying_q_positive_result.pdf}
          \caption{Positive result, part 1~\cref{thm:clean}}
          \label{fig:clean_edges_varying_q_positive}
      \end{subfigure}
      \begin{subfigure}[b]{0.49\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{figures/clean_edges_varying_q_negative_result.pdf}
          \caption{Negative result, part 2~\cref{thm:clean}}
          \label{fig:clean_edges_varying_q_negative}
      \end{subfigure}
      \caption{Demonstration of part 1 and 2 of~\cref{thm:clean}. }\label{fig:clean_edges_varying_q}
 \end{figure}

\textbf{Varying the distance of the means of the node features.} We illustrate how the attention coefficients and the accuracy change with the distance $\|\mu\|$. We fix $p=0.4$ and $q=0.33$ (this makes the graphs sufficiently noisy). We vary $\|\mu\|$ from $0.1\sigma \sqrt{\log n / (n\max(p,q))}$ to $20\sigma \sqrt{\log n}$. \cref{fig:clean_edges_varying_distance_gammas} illustrates~\cref{prop:gammas}. We observe empirically the separation of intra- and inter-$\gamma$ as claimed in~\cref{prop:gammas}. \cref{fig:clean_edges_varying_distance_accuracy} illustrates a combination of parts 1 and 2 of~\cref{thm:clean}. We observe that when the edge features are clean and $|p-q|$ is small then graph attention is better than graph convolution.
 \begin{figure}[ht!]
      \centering
      \begin{subfigure}[b]{0.49\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{figures/clean_edges_varying_distance_gammas.pdf}
          \caption{\cref{prop:gammas}}
          \label{fig:clean_edges_varying_distance_gammas}
      \end{subfigure}
      \begin{subfigure}[b]{0.49\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{figures/clean_edges_varying_distance_accuracy.pdf}
          \caption{Parts 1 and 2 of~\cref{thm:clean}}
          \label{fig:clean_edges_varying_distance_accuracy}
      \end{subfigure}
      \caption{This figure demonstrates how the attention coefficients and the accuracy are changing as a function of the distance between the means of the node features. }\label{fig:clean_edges_varying_distance}
 \end{figure}
 
\subsection{Noisy edge features}

We set $\zeta=0.1$ and we pick the mean of the edge features $\nu$ such that $\|\nu\|\ge 100 \zeta$.

\textbf{Varying $q$.} We fix $p=0.4$ and we vary $q$ from $\log^2/n$ to $2p$. We perform two experiments to demonstrate parts 1 and 2 of~\cref{thm:noisy}, For part 1, which is the positive result, we pick $\mu$ such that $\|\mu\| = 8\sigma \frac{p+q}{|p-q|}\sqrt{\log n / (n\max(p,q))}$. For part 2, which is the negative result, we set $\|\mu\| = 0.1\sigma \frac{p+q}{|p-q|}\sqrt{\log n / (n\max(p,q))}$. In~\cref{fig:noisy_edges_varying_q_positive} we present the positive result for graph attention and we also compare graph attention to graph convolution. We observe that for any value of $q$ graph attention has very similar performance to graph convolution. In~\cref{fig:noisy_edges_varying_q_negative} we present the negative result for graph attention. In this experiment, graph attention has very similar performance to graph convolution because the attention coefficients are approximately uniform.
 \begin{figure}[ht!]
      \centering
      \begin{subfigure}[b]{0.49\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{figures/noisy_edges_varying_q_positive_result.pdf}
          \caption{Positive result, part 1~\cref{thm:noisy}}
          \label{fig:noisy_edges_varying_q_positive}
      \end{subfigure}
      \begin{subfigure}[b]{0.49\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{figures/noisy_edges_varying_q_negative_result.pdf}
          \caption{Negative result, part 2~\cref{thm:noisy}}
          \label{fig:noisy_edges_varying_q_negative}
      \end{subfigure}
      \caption{Demonstration of part 1 and 2 of~\cref{thm:noisy}. }\label{fig:noisy_edges_varying_q}
 \end{figure}

\textbf{Varying the distance of the means of the node features.} In this experiment we illustrate how the attention coefficients and the accuracy change as a function of the distance $\|\mu\|$. We fix $p=0.4$ and $q=0.33$ (this makes the graphs sufficiently noisy). We vary $\|\mu\|$ from $0.01\sigma \frac{p+q}{|p-q|}\sqrt{\log n / (n\max(p,q))}$ to $20\sigma \sqrt{\log n}$. \cref{fig:noisy_edges_varying_distance_gammas} illustrates~\cref{prop:gammas_noisy}. We observe empirically that intra- and inter-$\gamma$ concentrate around the same value and they are both approximately uniform as claimed in~\cref{prop:gammas_noisy}. \cref{fig:noisy_edges_varying_distance_accuracy} illustrates a combination of parts 1 and 2 of~\cref{thm:noisy}. We observe that graph attention has very similar performance to graph convolution.
 \begin{figure}[ht!]
      \centering
      \begin{subfigure}[b]{0.49\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{figures/noisy_edges_varying_distance_gammas.pdf}
          \caption{\cref{prop:gammas_noisy}}
          \label{fig:noisy_edges_varying_distance_gammas}
      \end{subfigure}
      \begin{subfigure}[b]{0.49\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{figures/noisy_edges_varying_distance_accuracy.pdf}
          \caption{Parts 1 and 2 of~\cref{thm:noisy}}
          \label{fig:noisy_edges_varying_distance_accuracy}
      \end{subfigure}
      \caption{This figure demonstrates how the attention coefficients and the accuracy are changing as a function of the distance between the means of the node features. }\label{fig:noisy_edges_varying_distance}
 \end{figure}

\textbf{Attention coefficients for varying the distance of the means of the edge features.} In this experiment we demonstrate how the attention coefficients scale as a function of the distance between the means of the edge features. This is basically a combination of the results in~\cref{prop:gammas} and~\cref{prop:gammas_noisy}. We fix $p=0.4$ and $q=0.33$ (this makes the graphs sufficiently noisy). We vary $\|\nu\|$ from $0.01\zeta \sqrt{\log (0.5n^2(p+q))}$ to $30\zeta \sqrt{\log (0.5n^2(p+q))}$. The results are presented in~\cref{fig:varying_distance_of_edge_features_gammas}. We observe that for small distance between the means of the edge features the attention coefficients concentrate around the uniform measure, see~\cref{prop:gammas_noisy}, while as the distance increases then the intra-$\gamma$ increase up to the value $2/np$, see~\cref{prop:gammas} and the inter-$\gamma$ become very small, see~\cref{prop:gammas}. 

 \begin{figure}[ht!]
      \centering
      \begin{subfigure}[b]{0.5\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{figures/varying_distance_of_edge_features_gammas.pdf}
        %   \caption{\cref{prop:gammas} and \cref{prop:gammas_noisy}}
        %   \label{fig:varying_distance_of_edge_features_gammas}
      \end{subfigure}
      \caption{\cref{prop:gammas} and~\cref{prop:gammas_noisy}. }\label{fig:varying_distance_of_edge_features_gammas}
 \end{figure}
 
\section{Experiments on Real Data}

% In this experiment, we illustrate the performance of graph attention and graph convolution. We illustrate

We use the popular real data Amazon Computers, Amazon Photos, Cora, PubMed, and CiteSeer. These data are publicly available and can be downloaded from~\cite{FL2019}. The datasets come with multiple classes, however, for each of our experiments we do a one-v.s.-all  classification. This is a semi-supervised problem, only a fraction of the training nodes have labels. The rest of the nodes are used for measuring prediction accuracy. For Cora, PubMed and CiteSeer we use the train/test split that is given by~\cite{FL2019}. For Amazon Computers and Photos where the train/test split is not given we sample randomly $1\%$ of the nodes for training, the rest are used for testing. For each dataset we split the number of features into the first half and second half. The former is used for node features and the latter is used for edge features. The edge features are given by the concatenation of the features adjacent to the edge.\footnote{In the appendix we also show experiments without the feature split where all features are used as node features. In this case we use the concatenated edge features as described in the original paper~\cite{Velickovic2018GraphAN} and also in our Preliminaries section. We observe similar performance as in edge splitting.} We present results averaged over $5$ trials to account for randomness in initialization of parameters.

We observe that graph attention is giving similar attention mass to intra- and inter-edges as graph convolution which uses uniform weights as attention coefficients. This also explains the that there is no clear winner between graph attention and graph convolution when it comes to performance. In~\cref{table:1} we illustrate these observations. We present results for class $0$ and $1$ of each dataset. The experiments for the other classes are shown in the appendix. In~\cref{table:1} the intra-mass column is the percentage of the total probability mass assigned to intra-edges by intra-edge attention coefficients. Similarly for the inter-mass column. We observe that graph attention and graph convolution assign similar percentage of the mass to intra- and inter-edges. This results in graph attention performing similarly to graph convolution. We observe the same results for the rest of the classes in the appendix. It is important to mention that the attention coefficients of graph attention might not be exactly uniform or up to a constant uniform since our assumptions for CSBM might be violated, however, we still observe that graph attention has overall the same allocation of intra- and inter-mass to graph convolution. Finally, we observe that the majority of mass is assigned to intra-edges. This is expected since we are solving one-v.s.-all classification problems. However, we would still expect graph attention to have much better mass allocation for inter-edges than graph convolution, but it does not.

\begin{table}[ht!]
\caption{Percentages of intra- and inter-mass allocation for graph attention (GA) and graph convolution (GC), and test accuracy.} \vspace{0.1cm}
\centering
 \begin{tabular}{||c | c c c c c ||} 
 \hline
 data & class & method & intra-m & inter-m  & acc.\\ [0.5ex] 
 \hline\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{Amzn Co.}} & \multirow{2}{*}{$0$} & GC & $98.7$ & $1.3$ & $96.8$ \\
& & GA & $98.1$ & $1.9$ & $96.7$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $93.6$ & $6.4$ & $91.4$ \\
& & GA & $93.3$ & $6.7$ & $88.7$ \\
\hline \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{Amzn Ph.}} & \multirow{2}{*}{$0$} & GC & $99.0$ & $1.0$ & $95.1$ \\
& & GA & $98.8$ & $1.2$ & $96.0$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $94.9$ & $5.1$ & $94.2$ \\
& & GA & $95.5$ & $4.5$ & $89.0$ \\
\hline \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{Cora}} & \multirow{2}{*}{$0$} & GC & $94.2$ & $5.8$ & $89.5$ \\
& & GA & $94.7$ & $5.3$ & $88.6$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $97.3$ & $2.7$ & $92.3$ \\
& & GA & $97.4$ & $2.6$ & $93.7$ \\
\hline \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{PubMed}} & \multirow{2}{*}{$0$} & GC & $92.2$ & $7.8$ & $82.1$ \\
& & GA & $92.1$ & $7.9$ & $82.8$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $91.4$ & $8.6$ & $58.8$ \\
& & GA & $90.6$ & $9.4$ & $59.5$ \\
\hline \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{CiteSeer}} & \multirow{2}{*}{$0$} & GC & $94.3$ & $5.7$ & $92.0$ \\
& & GA & $94.4$ & $5.6$ & $91.6$ \\ \cline{2-6}
& \multirow{2}{*}{$1$} & GC & $92.6$ & $7.4$ & $82.6$ \\
& & GA & $92.8$ & $7.2$ & $82.8$ \\
\hline 
\end{tabular}
\label{table:1}
\end{table}

==> On Classification Thresholds for Graph Attention with Edge Features (arXiv)/packages.tex <==
\usepackage{geometry}
%
\geometry{letterpaper,margin=1in}
\usepackage{subcaption}
\usepackage{cite}
\usepackage{xspace}
\usepackage{booktabs} % for professional tables
\usepackage[toc,page]{appendix}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{mathtools} % An extension package to amsmath
\usepackage{comment}
\usepackage{multirow}
\usepackage{multicol}
\usepackage[export]{adjustbox}
 \usepackage{array}
 \usepackage{arydshln}
 \usepackage{makecell}
 \usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{enumitem}
\usepackage{xcolor}

\usepackage{apptools}
\AtAppendix{\counterwithin{theorem}{section}} % numbering theorems/lemmas in Appendix by section A, B, C, ...

%\usepackage{fullpage}
\usepackage{comment}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage{multirow}
% \usepackage{authblk}
\usepackage{dsfont}
\usepackage{breakcites}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{caption}
% \usepackage{paralist}
\usepackage{subcaption}
\usepackage{latexsym,bbm,graphicx,float,mathtools}

\usepackage[colorlinks,linkcolor=blue,citecolor=blue]{hyperref}
% \usepackage{url}
\usepackage[capitalize,nameinlink]{cleveref}
% \usepackage[hang,flushmargin]{footmisc}
